Multinomial, Poisson and Gaussian statistics in count data analysis

It is generally known that counting statistics is not correctly described by a Gaussian approximation. Nevertheless, in neutron scattering, it is common practice to apply this approximation to the counting statistics; also at low counting numbers. We show that the application of this approximation leads to skewed results not only for low-count features, such as background level estimation, but also for its estimation at double-digit count numbers. In effect, this approximation is shown to be imprecise on all levels of count. Instead, a Multinomial approach is introduced as well as a more standard Poisson method, which we compare with the Gaussian case. These two methods originate from a proper analysis of a multi-detector setup and a standard triple axis instrument.We devise a simple mathematical procedure to produce unbiased fits using the Multinomial distribution and demonstrate this method on synthetic and actual inelastic scattering data. We find that the Multinomial method provide almost unbiased results, and in some cases outperforms the Poisson statistics. Although significantly biased, the Gaussian approach is in general more robust in cases where the fitted model is not a true representation of reality. For this reason, a proper data analysis toolbox for low-count neutron scattering should therefore contain more than one model for counting statistics.

==> unused.tex <==
{\color{red}
\iffalse
The other three parameters seem to be correlated in their determination. All of the methods overestimates the amplitude, $\langle A_{\rm est} \rangle$, especially all of the $\chi^2$ methods for almost all background levels. Further, the background estimate, $\langle B_{\rm est} \rangle$, is underestimated to different degrees. 



%Unlike for the peak center, the estimation of the peak width is affected by the background level for the Gaussian least squares fits, and it is underestimated (by up to 10\%) by all three methods for low background values up to a value of $B \leq 3$, but overestimated by 1-2\% for $B \geq 6$. In contrast, the Poisson fits nicely reproduce the model width of $\langle \sigma_{\rm est} \rangle = 0.100$.
%This wrong estimation of the peak width by the Gaussian methods is rather curious. From the fit to the pure background model we saw that the estimated $B$ was held low due to larger confidence being given to (accidental) low count data. In a naive view, such an effect could cause an average peak narrowing due to random low-count events on the wings of the peak. In contrast, we observe the opposite. At present, we cannot explain this fully in detail.

It is somewhat surprising that the estimation the peak amplitude, $\langle A_{\rm est} \rangle$, is systematically too high, even for the Poisson statistics. In particular for the Poisson method, since this has proven to be very robust in the estimations of background level. Depending on the background level, $\langle A_{\rm est} \rangle$ is as much as 0.5 too high for the Poisson and 0.9 for the best Gaussian. In contrast, the background, $B$, is slightly underestimated for all methods. It can be seen that the amplitude and background estimations are coupled to the determination of the peak width. The fitting routines all try to compensate the over- and underestimation of the amplitude and background respectively by widening of the peak, i.e. $\langle \sigma_{\rm est}\rangle$. This ensures that the integrated intensity of the fit better resembles that of the data. The estimation of the peak width is affected by the background level for the Gaussian least squares fits: It is underestimated (by up to 10\%) by all three methods for low background values up to a value of $B \leq 3$, but overestimated by 1-2\% for $B \geq 6$. In contrast, the Poisson fits nicely reproduce the model width of $\langle \sigma_{\rm est} \rangle = 0.100$. However, almost across all background levels the Poisson underestimates it ever so slightly.

To investigate this coupling between number of points and parameter estimation further, we have performed the same simulations and fits for data series with $N=201$ and $N=21$ data points, as seen in Fig.~\ref{fig:NumerousRarePeakAmplitude}. This was performed so as to investigate if the above deviation merely reflects an uncertainty originating from limiting the number of data points in the peak. In the high point density limit, the Poisson fits converges better to the true amplitude across all background levels with a small overestimation of less than 0.5\%. 
In the other extreme, with a low number of data points, the seen overestimation of $\langle A_{\rm est} \rangle$ becomes larger together with the underestimation of $\langle B_{\rm est} \rangle$.

The estimates of the three other model parameters are largely unchanged by the additional amounts of data, except that the standard deviations of the estimated parameters are lowered by about a factor of 2, which could be expected from the general $1/\sqrt{N}$ law. 


\begin{figure}[h!]
    \centering
    \textbf{$N=201$}\par\medskip
    \includegraphics[width=0.45\linewidth]{PDFfigures/Peak_A_numerous}
    \includegraphics[width=0.45\linewidth]{PDFfigures/Peak_B_numerous}\\
    \textbf{$N=21$}\par\medskip
    \includegraphics[width=0.45\linewidth]{PDFfigures/Peak_A_lowLimit}
    \includegraphics[width=0.45\linewidth]{PDFfigures/Peak_B_lowLimit}
    \caption{\textbf{Top}: Statistics of fits to data sets with 201 data points in the range from -1.0 to 1.0. \textbf{Bottom}: Statistics of fits to data sets with 21 data points in the range from -0.5 to 0.5. \textbf{Left}: Fitted peak amplitude. \textbf{Right}: Fitted background level. }
    \label{fig:NumerousRarePeakAmplitude}
\end{figure}
\fi
}

Further, curves for constant log likelihood can also be plotted, and an example for the four previously described methods is shown in Fig.~\ref{fig:ErrorEstimateMinuit} for a Gaussian peak shape of height 20 on a constant background of 16 counts. Fig.~\ref{fig:ErrorEstimateHistogram} shows the correlation between $\langle A_{\rm est} \rangle$ and $\langle B_{\rm est} \rangle$ for only the Poisson and $\chi^2$ methods, at low background level. It is clear that only the Poisson method truly fits the data, while all the $\chi^2$ methods are multiple standard deviations away.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.75\linewidth]{PDFfigures/ErrorEstimate_16}
    \caption{Estimated $1\sigma$, $2 \sigma$, and $3 \sigma$ confidence intervals for the amplitude ($A$) and background ($B$) fitting parameters for one synthetic data set from a model with a Gaussian peak on constant background as described in section~\ref{sect:simplemodels}. The value of the true model parameters are displayed as a black dot in each panel at the point $(A,B) = (20,16)$. 
    }
    \label{fig:ErrorEstimateMinuit}
\end{figure}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.45\linewidth]{PDFfigures/PeakScatterPlotPoisson_2_0}
    \includegraphics[width=0.45\linewidth]{PDFfigures/PeakScatterPlotchi2BG1_2_0}
    \includegraphics[width=0.45\linewidth]{PDFfigures/PeakScatterPlotchi2BG2_2_0}
    \includegraphics[width=0.45\linewidth]{PDFfigures/PeakScatterPlotchi2BG3_2_0}
    \caption{Scatter plot of parameters determined from a series of synthetic data sets, using the four different methods, plotted together with histograms of distribution of the fitted value background and amplitude, their true parameters being $B$ = 2.0 and $A$ = 20.0. The 1, 2, and 3 $\sigma$ co-variances are plotted as ellipses, while the true and average fitted parameter estimates are signified by a cross and an empty circle, respectively.}
    \label{fig:ErrorEstimateHistogram}
\end{figure}

